A Comparative Attention Framework for Better Few-Shot Object Detection on Aerial Images

Few-Shot Object Detection (FSOD) methods are mainly designed and evaluated on natural image datasets such as Pascal VOC and MS COCO. However, it is not clear whether the best methods for natural images are also the best for aerial images. Furthermore, direct comparison of performance between FSOD methods is difficult due to the wide variety of detection frameworks and training strategies. Therefore, we propose a benchmarking framework that provides a flexible environment to implement and compare attention-based FSOD methods. The proposed framework focuses on attention mechanisms and is divided into three modules: spatial alignment, global attention, and fusion layer. To remain competitive with existing methods, which often leverage complex training, we propose new augmentation techniques designed for object detection. Using this framework, several FSOD methods are reimplemented and compared. This comparison highlights two distinct performance regimes on aerial and natural images: FSOD performs worse on aerial images. Our experiments suggest that small objects, which are harder to detect in the few-shot setting, account for the poor performance. Finally, we develop a novel multiscale alignment method, Cross-Scales Query-Support Alignment (XQSA) for FSOD, to improve the detection of small objects. XQSA outperforms the state-of-the-art significantly on DOTA and DIOR.

==> Parts/16_rmap_xqsa.tex <==
\section{Cross-scales Query-Support Alignment RmAP Analysis}
\label{app:rmap_all}
In order to assess how well the XQSA method performs on aerial and
natural images, we present in \cref{fig:rmap_all_hist} an extended version of
the plot from \cref{fig:baseline_res} with DANA and XQSA. The exact values of
mAP and RmAP are regrouped in \cref{tab:rmap_values}. This summarizes the
conclusions from \cref{sec:xscale}, XQSA improves largely over the previous
methods on DOTA and DIOR. However, there remains a large performance gap
compared to the no few-shot baseline, i.e. the RmAP (white percentage values on
the bar chart) is still low compared with RmAP on natural images. 
%



\begin{table}[h]
\centering
\caption{$\text{mAP}_{0.5}$ and RmAP values for some reimplemented methods
and XQSA with $K=10$ shots. These are the values used to make the plot from
\cref{fig:rmap_all_hist}}
\label{tab:rmap_values}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{@{}llccccccccl@{}}
\toprule[1pt]
                                &               & \multicolumn{2}{c}{\textbf{DOTA}} &  & \multicolumn{2}{c}{\textbf{DIOR}} & \textbf{} & \multicolumn{2}{c}{\textbf{Pascal VOC}} &  \\
                                &               & \textbf{Base}   & \textbf{Novel}  &  & \textbf{Base}   & \textbf{Novel}  &           & \textbf{Base}      & \textbf{Novel}     &  \\ \cmidrule(r){1-10}
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{$\text{mAP}_{\mathbf{0.5}}$}}}  & FCOS baseline & 0.61            & 0.70            &  & 0.73            & 0.82            &           & 0.66               & 0.68               &  \\ \cmidrule(lr){2-10}
                                & FRW           & 0.49            & 0.35            &  & 0.61            & 0.37            &           & 0.63               & 0.49               &  \\
                                & WSAAN         & 0.47            & 0.35            &  & 0.63            & 0.32            &           & 0.65               & 0.52               &  \\
                                & DANA          & 0.54            & 0.37            &  & 0.63            & 0.38            &           & 0.65               & 0.52               &  \\
                                & XQSA          & 0.51            & 0.41            &  & 0.60            & 0.42            &           & 0.51               & 0.47               &  \\
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{RmAP (\%)}}}                               &               &                 &                 &  &                 &                 &           &                    &                    &  \\
                                & FRW           & -19.43          & -49.36          &  & -15.83          & -54.23          &           & -3.52              & -28.39             &  \\
                                & WSAAN         & -23.24          & -49.60          &  & -13.78          & -60.26          &           & -0.30              & -24.00             &  \\
                                & DANA          & -11.30          & -47.63          &  & -13.88          & -53.14          &           & -0.46              & -23.17             &  \\
                                & XQSA          & -16.03          & -41.17          &  & -17.78          & -49.05          &           & -21.97             & -31.39             &  \\ \bottomrule[1pt]
\end{tabular}%
}
\end{table}

\newpage

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.95\columnwidth]{Figures/fig_dataset_comparison_all_methods_vertical.png}
    \caption{$\text{mAP}_{0.5}$ and corresponding RmAP values of the four best performing
    methods from all our experiments. All methods are trained within our
    proposed AAF framework with data augmentation which explains slightly
    higher performance for FRW and WSA. 10 shots are available for each
    class at inference time.}
    \label{fig:rmap_all_hist}
\end{figure}


